Policy-Compliant Path Diversity and Bisection Bandwidth

How many links can be cut before a network is bisected? What is the maximal bandwidth that can be pushed between two nodes of a network? These questions are closely related to network resilience, path choice for multipath routing or bisection bandwidth estimations in data centers. The answer is quantified using metrics such as the number of edge-disjoint paths between two network nodes and the cumulative bandwidth that can flow over these paths. In practice though, such calculations are far from simple due to the restrictive effect of network policies on path selection. Policies are set by network administrators to conform to service level agreements, protect valuable resources or optimize network performance. In this work, we introduce a general methodology for estimating lower and upper bounds for the policy-compliant path diversity and bisection bandwidth between two nodes of a network, effectively quantifying the effect of policies on these metrics. Exact values can be obtained if certain conditions hold. The approach is based on regular languages and can be applied in a variety of use cases.

==> Makefile <==
## Fully automated LaTeX Makefile
## (c) Bernhard Ager 2010
## Released under GPLv3 <http://www.gnu.org/licenses/gpl.txt>
##
## This is supposed to work with no (or at most a few) modifications 
## on any LaTeX source directory as a drop in.
## 
## If you have suggestions for or additions to this Makefile, feel free to
## drop me <bernhard@net.t-labs.tu-berlin.de> a mail. I am especially
## interested in further/better auto-conversion rules for picture formats.
##
## Acknowledgements go to Oliver Hohlfeld for proposing a database to track
## auto-generated pictures.
##
## Hard dependencies: GNU make, sed, grep, rm
## Soft dependencies: the tools to convert to the different formats including
## latex, pdflatex, dvips, pstopdf, eps2pdf, fig2dev, inkscape, wmf2eps, ...


## $(MAIN).tex is assumed to be the main latex file
MAIN=$(basename $(shell grep -Fl '\documentclass' *.tex))

## $(TEXFILES) holds all LaTeX source files. Extend wildcard pattern if you
## are holding tex files in subdirectories or adjust to your needs.
TEXFILES=$(wildcard *.tex)

## $(PICTURES) and $(BIBLIOGRAPHY) try to guess the names of required 
## pictures and bib files. The matching rule is quite primitive and is
## easily confused by clutter in lines with \includegraphics or 
## \bibliography. 
PICTURES=$(shell grep -F '\includegraphics' $(TEXFILES) | \
		grep -v '%.*\\includegraphics' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfimage' $(TEXFILES) | \
		grep -v '%.*\\pgfimage' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfdeclareimage' $(TEXFILES) | \
		grep -v '%.*\\pgfdeclareimage' | sed 's/.*{\([^{}]*\)}.*/\1/')

BIBLIOGRAPHY=$(addsuffix .bib, $(shell grep -F '\bibliography{' $(TEXFILES) | \
	grep -v '%.*\\bibliography' | sed 's/.*{\([^{}]*\)}.*/\1/'))

PS_PICTURES=$(addsuffix .eps, $(PICTURES))
PDF_PICTURES=$(addsuffix .pdf, $(PICTURES))

## $(PICTURE_DB) keeps track of which pictures were actually created by
## this Makefile. In the clean target this database is used to remove them.
## You might have some manual work to do if you accidentially remove it.
PICTURE_DB = picture.db
PICTURE_DB_ADD = test -f $(PICTURE_DB) && grep -F "$@" $(PICTURE_DB) || echo "$@" >>$(PICTURE_DB)

PDFTK=/usr/bin/pdftk

## call pdflatex target if you prefer pdflatex over latex, dvips, ps2pdf
#
all: pdflatex
# all: $(MAIN).pdf
# all: pdflatex # $(MAIN).ps $(MAIN).pdf
# all: $(MAIN).pdf

## Detection of changed '\cite'ations is a PITA. Any hints welcome.
pdflatex: $(MAIN).tex $(TEXFILES) $(PDF_PICTURES) $(BIBLIOGRAPHY)
	pdflatex $<
ifneq ($(BIBLIOGRAPHY), )
	bibtex $(MAIN) && pdflatex $< && pdflatex $<
endif
	test -f $(PDFTK) && $(PDFTK) $(MAIN).pdf output $(MAIN)_out.pdf compress || cp $(MAIN).pdf $(MAIN)_out.pdf

.PHONY: $(MAIN).ps $(MAIN).pdf $(MAIN).dvi

$(MAIN).ps: $(MAIN).dvi
	dvips -z -P pdf -t letter -o $@ $<

$(MAIN).pdf: $(MAIN).ps
	ps2pdf -dSAFER -dNOPLATFONTS -dEmbedAllFonts#true -dPDFSETTINGS#/prepress $< $@

## Detection of changed '\cite'ations is a PITA. Any hints welcome.
$(MAIN).dvi: $(MAIN).tex $(TEXFILES) $(PS_PICTURES) $(MAIN).bbl
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).oc
	latex $<
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).nc
	cmp $(MAIN).oc $(MAIN).nc || bibtex $(MAIN) && latex $< && latex $<

$(MAIN).bbl: $(BIBLIOGRAPHY)
	latex $(MAIN).tex
	bibtex $(MAIN).aux || true
	latex $(MAIN).tex

## unfortunately produces broken pictures, fallback to eps and eps2pdf
#%.pdf: %.dia
#	dia --export=$@ $<
#	$(PICTURE_DB_ADD)

#%.eps: %.dia
#	dia --export=$@ $<
#	$(PICTURE_DB_ADD)

%.pdf: %.fig
	fig2dev -L pdf $< $@
	$(PICTURE_DB_ADD)

%.eps: %.fig
	fig2dev -L eps $< $@
	$(PICTURE_DB_ADD)

%.eps: %.jpg
	convert $< $@
	$(PICTURE_DB_ADD)

%.eps: %.png
	convert $< $@
	$(PICTURE_DB_ADD)

%.pdf: %.svg
	inkscape --export-pdf=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.svg
	inkscape --export-eps=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.wmf
	wmf2eps --eps -o $@ $<
	$(PICTURE_DB_ADD)

# this rule requires the R script to plot to the correct file,
# relative to the Makefile!
%.eps: %.R
	R --no-save <$<
	test -f $@
	test $@ -nt $<

## This generic rule should be kept as the last one, so that
## native -> pdf generation takes precedence over native -> eps -> pdf
#%.pdf: %.eps
#	epstopdf --outfile=$@ $<
#	$(PICTURE_DB_ADD)

%.eps: %.pdf
	pdftops -eps $< $@
	$(PICTURE_DB_ADD)

clean:
	rm -f $(MAIN).aux $(MAIN).dvi $(MAIN).log $(MAIN).nav $(MAIN).out \
		$(MAIN).pdf $(MAIN).ps $(MAIN).snm $(MAIN).toc $(MAIN).bbl \
		$(MAIN).blg $(MAIN).oc $(MAIN).nc head.tmp body.tmp
	rm -f $(shell test -f $(PICTURE_DB) && cat $(PICTURE_DB))
	rm -f $(PICTURE_DB)

